Markerless Robot Detection and 6D Pose Estimation for Multi-Agent SLAM

The capability of multi-robot SLAM approaches to merge localization history and maps from different observers is often challenged by the difficulty in establishing data association. Loop closure detection between perceptual inputs of different robotic agents is easily compromised in the context of perceptual aliasing, or when perspectives differ significantly. For this reason, direct mutual observation among robots is a powerful way to connect partial SLAM graphs, but often relies on the presence of calibrated arrays of fiducial markers (e.g., AprilTag arrays), which severely limits the range of observations and frequently fails under sharp lighting conditions, e.g., reflections or overexposure. In this work, we propose a novel solution to this problem leveraging recent advances in Deep-Learning-based 6D pose estimation. We feature markerless pose estimation as part of a decentralized multi-robot SLAM system and demonstrate the benefit to the relative localization accuracy among the robotic team. The solution is validated experimentally on data recorded in a test field campaign on a planetary analogous environment.

==> tables/sim_summary_order1_colorful.tex <==

\begingroup



\definecolor{ValuePurple}{rgb}{0.2, 0.1, 1.0}
\definecolor{ValueBlue}{rgb}{0.2, 0.6, 0.8}
\definecolor{ValueGreen}{rgb}{0.2, 0.8, 0.3}

%\definecolor{ValueGreen}{rgb}{0.3, 0.3, 0.8}

\colorlet{LightPurple}{ValuePurple!11}  \colorlet{LightBlue}{ValueBlue!13}  \colorlet{LightGreen}{ValueGreen!13}
\colorlet{MidPurple}{ValuePurple!32}    \colorlet{MidBlue}{ValueBlue!32}    \colorlet{MidGreen}{ValueGreen!33}
\colorlet{DarkPurple}{ValuePurple!52}   \colorlet{DarkBlue}{ValueBlue!58}   \colorlet{DarkGreen}{ValueGreen!59}   

\setlength{\tabcolsep}{2.5pt}
\renewcommand{\arraystretch}{1.43}

% Requires: \usepackage{multirow}
\begin{table}[tp!]
    \centering
    \captionsetup{justification=centering}
    \caption{Synthetic Test Results: Detection rate $\rho$, translation error $t$, rotational error $\theta$ for different training and test set combinations.
    The arrow after a variable indicates whether a higher ($\uparrow$) or lower ($\downarrow$) value is desirable.}
    \label{tab:results:simulation_results_order1_colorful}
    \renewcommand{\arraystretch}{1}
    \resizebox{\linewidth}{!}{
    \begin{tabularx}{\linewidth}{|c|c|c|Y|Y|Y|}
        \hline
        %& & & & & \\
        \footnotesize
        \makecell{\textbf{Training} \\ \textbf{Set}} & \makecell{\textbf{Test} \\ \textbf{Set}} & \makecell{\textbf{Observed} \\ \textbf{Robot}} & $\rho\ (\uparrow)$ & $t\ [m]\ (\downarrow)$ & $\theta\ [rad]\ (\downarrow)$ \\%[2ex]
        \hline
        \multirow{4}{*}{BPROC} & \multirow{2}{*}{BPROC} & Lander & \cellcolor{LightPurple}0.160 & \cellcolor{MidBlue}0.310 & \cellcolor{DarkGreen}\textbf{0.421} \\ \hhline{~~----}
        & & LRU & \cellcolor{MidPurple}0.080 & \cellcolor{DarkBlue}\textbf{0.082} & \cellcolor{DarkGreen}\textbf{0.099} \\ \hhline{~-----}
        & \multirow{2}{*}{OAISYS} & Lander & \cellcolor{LightPurple}0.080 & \cellcolor{LightBlue}0.184 & \cellcolor{LightGreen}0.483 \\ \hhline{~~----}
        & & LRU & \cellcolor{LightPurple}0.020 & \cellcolor{DarkBlue}\textbf{0.034} & \cellcolor{LightGreen}0.128 \\ \hline
        \multirow{4}{*}{\textbf{OAISYS}} & \multirow{2}{*}{BPROC} & Lander & \cellcolor{MidPurple}0.260 & \cellcolor{LightBlue}1.497 & \cellcolor{LightGreen}2.207 \\ \hhline{~~----}
        & & LRU & \cellcolor{LightPurple}0.064 & \cellcolor{LightBlue}1.621 & \cellcolor{LightGreen}1.143 \\ \hhline{~-----}
        & \multirow{2}{*}{OAISYS} & Lander & \cellcolor{MidPurple}0.676 & \cellcolor{MidBlue}0.044 & \cellcolor{MidGreen}0.089 \\ \hhline{~~----}
        & & LRU & \cellcolor{MidPurple}0.184 & \cellcolor{LightBlue}0.115 & \cellcolor{MidGreen}0.092 \\ \hline
        \multirow{4}{*}{\textbf{COMBINED}} & \multirow{2}{*}{BPROC} & Lander & \cellcolor{DarkPurple}\textbf{0.284} & \cellcolor{DarkBlue}\textbf{0.259} & \cellcolor{MidGreen}0.514 \\ \hhline{~~----}
        & & LRU & \cellcolor{DarkPurple}\textbf{0.324} & \cellcolor{MidBlue}0.153 & \cellcolor{MidGreen}0.188 \\ \hhline{~-----}
        & \multirow{2}{*}{OAISYS} & Lander & \cellcolor{DarkPurple}\textbf{0.792} & \cellcolor{DarkBlue}\textbf{0.040} & \cellcolor{DarkGreen}\textbf{0.048} \\ \hhline{~~----}
        & & LRU & \cellcolor{DarkPurple}\textbf{0.764} & \cellcolor{MidBlue}0.098 & \cellcolor{DarkGreen}\textbf{0.052} \\ \hline
    \end{tabularx}}
\end{table}
\endgroup


==> tables/slam_performance_3_runs_combined.tex <==
\begingroup
\setlength{\tabcolsep}{1.8pt}
\begin{table}[!tp]
\caption{Multi-robot SLAM performance of the real-world outdoor mission data with limited input knowledge (AprilTag) compared to full input knowledge (AprilTag + Markerless) \todo{Can we also add the number of robot detection events, and show an improvement there? }}
\label{tab:combined_slam_error}
\centering
\renewcommand{\arraystretch}{1.1}
\resizebox{\linewidth}{!}{
\begin{tabular}{l c c c c}
\hline
\textbf{Modality} & \textbf{Traj. Error} & \makecell{\textbf{Max Det.} \\ \textbf{Distance}} & \makecell{\textbf{Max Open-} \\ \textbf{Loop Duration}}  & \textbf{\# Detections}\\
\hline
\multicolumn{4}{c}{\textbf{Mission 1}} \\
Fid.               & 0.83m & 5.00m & 936s & 262 \\ %71+191(LRU+LRU2) \\ %123+510(tags)\\
Fid. + Markerl.  & 0.55m & 5.78m & 621s & 273 \\ %77+196(LRU+LRU2) \\ %129+515(tags)\\
\hline
Improvement             & \dgreen{\textbf{-34\%}} & \dgreen{\textbf{+16\%}} & \dgreen{\textbf{-34\%}} & \dgreen{\textbf{+4\%}} \\
\hline
\multicolumn{4}{c}{\textbf{Mission 2}} \\
%\textbf{Input Knowledge} & \textbf{Localization Accuracy} & \textbf{Observable Distance} & \textbf{Longest Open-Loop Navigation} \\
Fid.               & 1.00m & 5.63m & 2300s & 203 \\ %49+154(LRU+LRU2) \\ %189+281(tags)\\
Fid. + Markerl.  & 0.79m & 16.15m & 1033s & 267 \\ %87+180(LRU+LRU2) \\ %227+307(tags)\\
\hline
Improvement             & \dgreen{\textbf{-22\%}} & \dgreen{\textbf{+186\%}} & \dgreen{\textbf{-55\%}} & \dgreen{\textbf{+32\%}} \\
\hline
\multicolumn{4}{c}{\textbf{Mission 3}} \\
%\textbf{Input Knowledge} & \textbf{Localization Accuracy} & \textbf{Observable Distance} & \textbf{Longest Open-Loop Navigation} \\
Fid.               & 0.73m & 7.63m & 490s & 32 \\ %14+18(LRU+LRU2) \\ %30+21(tags)\\
Fid. + Markerl.  & 0.70m & 17.14m & 490s & 39 \\ %20+19(LRU+LRU2) \\ %36+22(tags\\
\hline
Improvement             & \dgreen{\textbf{-4\%}}   & \dgreen{\textbf{+125\%}} & \textbf{--} & \dgreen{\textbf{+22\%}} \\
\hline
\end{tabular}}
\end{table}
\endgroup
